Few-shot Segmentation with Optimal Transport Matching and Message Flow

We tackle the challenging task of few-shot segmentation in this work. It is essential for few-shot semantic segmentation to fully utilize the support information. Previous methods typically adopt masked average pooling over the support feature to extract the support clues as a global vector, usually dominated by the salient part and lost certain essential clues. In this work, we argue that every support pixel's information is desired to be transferred to all query pixels and propose a Correspondence Matching Network (CMNet) with an Optimal Transport Matching module to mine out the correspondence between the query and support images. Besides, it is critical to fully utilize both local and global information from the annotated support images. To this end, we propose a Message Flow module to propagate the message along the inner-flow inside the same image and cross-flow between support and query images, which greatly helps enhance the local feature representations. Experiments on PASCAL VOC 2012, MS COCO, and FSS-1000 datasets show that our network achieves new state-of-the-art few-shot segmentation performance.

==> Figures/VOC-qr.tex <==
 \begin{figure*}[t]
  \centering
    \includegraphics[width=1\linewidth]{Images/voc_qr.pdf}
    \caption{Our qualitative examples on the PASCAL VOC 2012 dataset. The left column is the prediction, and the right column is the ground truth.}
    \label{voc-qr}
\end{figure*}

==> Figures/fss-1000-qr.tex <==
 \begin{figure*}[t]
  \centering
    \includegraphics[width=1\linewidth]{Images/fss1000-qr.pdf}
    \caption{Our qualitative examples on the FSS-1000 dataset. The left column is the prediction, and the right column is the ground truth.}
    \label{fss1000-qr}
\end{figure*}

==> Figures/partial-show.tex <==
 \begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{Images/partial-show.pdf}
    \caption{Visualization of the partial optimal matching flows. Given two images (left and right), we plot the best-matched patch of each local region.}
    \label{partial show}
\end{figure}

==> Tables/coco-iou.tex <==

\begin{table}[t]
\centering
\small
\caption{Comparison with the state-of-the-art methods under the 1-shot and 5-shot setting. Our proposed network outperforms all previous methods and achieves new state-of-the-art performance. The results are reported on the MS COCO dataset with FBIoU(\%).}
\resizebox{0.7\columnwidth}{!}
{

\begin{tabular}{lcc}
\toprule[1pt]
Method & 1-shot (\%) & 5-shot (\%) \\
\hline
PANET \cite{wang2019panet}       & 59.2    & 63.5          \\
A-MCG \cite{hu2019attention}   & 52.0      & 54.7         \\
\hline
Ours     & \textbf{58.2}    & \textbf{59.6}     \\
\bottomrule[1pt]
\end{tabular}

}
\label{table-coco-bfiou}
\end{table}

==> Tables/partial-cos.tex <==

\begin{table}[t]
\centering
\small
\caption{Comparison our partial optimal layer and the cosine similarity under the 1-shot. Our proposed partial optimal layer can achieve better results. The results are reported on PASCAL VOC 2012 dataset with standard mIoU(\%) under the 1-shot setting.}
\resizebox{1\columnwidth}{!}
{
\begin{tabular}{lccccc}
\toprule[1pt]
Method & split-0 & split-1 & split-2 & split-3 & mean \\
\hline
Baseline     & 62.9   & 69.7  &55.8  & 56.7  &61.1        \\
Cosine     & 64.8    & 70.9  &55.4  & 57.0  &62.0        \\
Partial     & 65.4   & 71.5   &55.2   & 58.1   &62.5        \\
\bottomrule[1pt]
\end{tabular}

}
\label{table: partial-cos}
\end{table}
